FreqRISE: Explaining time series using frequency masking

Time-series data are fundamentally important for many critical domains such as healthcare, finance, and climate, where explainable models are necessary for safe automated decision making. To develop explainable artificial intelligence in these domains therefore implies explaining salient information in the time series. Current methods for obtaining saliency maps assume localized information in the raw input space. In this paper, we argue that the salient information of a number of time series is more likely to be localized in the frequency domain. We propose FreqRISE, which uses masking-based methods to produce explanations in the frequency and time-frequency domain, and outperforms strong baselines across a number of tasks. The source code is available here: \url{https://github.com/theabrusch/FreqRISE}.

==> files/app_postprocess.tex <==
\subsection{Post-processing of FreqRISE relevance maps}
We do some preliminary experiments to reduce the complexity of the FreqRISE relevance maps through thresholding. Due to the properties of LRP and IG, both methods are able to assign zero relevance to specific points in the input space. This is not the case for FreqRISE, due to the weighted average with which the relevance maps are computed. 

We post-process the FreqRISE results through thresholding.
Given a relevance map $\boldsymbol{R}_c$, we produce a post-processed relevance map $\boldsymbol{R}_c^p$ by computing the $p$-th quantile, $q_p$ and setting all elements, $\lambda$, with value below $q_p$ to 0:
\begin{equation}
    \boldsymbol{R}^p_c(\lambda) = \begin{cases}
    \boldsymbol{R}^p_c(\lambda), & \text{if $\boldsymbol{R}^p_c(\lambda)\geq q_p$}.\\
    0, & \text{otherwise}.
  \end{cases}
\end{equation}
We compare the faithfulness and complexity trade-off for post-processed relevance maps of FreqRISE with different thresholds $p$. 
% \begin{table}[h]
%     \centering
%     %\small
%     \caption{AudioMNIST: Faithfulness (F) and complexity (C) of explanations in the frequency (Freq.) and time-frequency (Time-freq.) domain.}
%     \begin{tabular}{lrrrrrrrr}
%          \toprule
%         & \multicolumn{4}{c}{Digit ($\downarrow$)} & \multicolumn{4}{c}{Gender ($\downarrow$)} \\
%         \cmidrule(r){2-5}\cmidrule{6-9}
%         &  \multicolumn{2}{c}{Freq.} & \multicolumn{2}{c}{Time-freq.} & \multicolumn{2}{c}{Freq.} & \multicolumn{2}{c}{Time-freq.}\\ 
%         & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{C}& \multicolumn{1}{c}{F} & \multicolumn{1}{c}{C}& \multicolumn{1}{c}{F} & \multicolumn{1}{c}{C} \\ \hline 
%         IG & $.251$ & $8.29$ & $.194 $& $8.26$ & $.428$ & $8.28$ & $\mathbf{.389}$ & $8.25$ \\
%         LRP & $.204$ & $8.25$ & $.209$ & $8.22$ & $.431$ & $7.73$ &$.420$ & $7.73$\\ \hline
%         IG$_{pos}$ & $.231$ & $6.41$ & $.192 $& $5.26$ & $.436$ & $4.74$ & $.405$ & $4.04$ \\
%         LRP$_{pos}$ & $.203$ & $5.84$ & $.202$ & $4.67$ & $.439$ & $5.16$ &$.429$ & $4.16$\\ \bottomrule
%     \end{tabular}
%     \label{tab:app_lrpig}
% \end{table}
Additionally, IG and LRP are both able to assign negative relevance to specific points. However, often when visualizing the relevance maps, negative values will be set to zero \cite{vilrp}. In the main paper, we set negative values to zero when evaluating the complexity, but not when evaluating the faithfulness, giving both baseline methods an advantage in either case. Here, we therefore include LRP and IG results when setting all negative values to 0 (LRP pos. and IG pos.) and when considering positive and negative values (LRP and IG). 

On the synthetic dataset, we set $p=0.997$ and achieve a complexity score of 1.17 for both the low noise and high noise setting, while maintaining a localization score of 100\% on both tasks. 

All results are visualized in \autoref{fig:comp_vs_faith}.

\begin{figure}[h]
    \centering
    \includegraphics{figs/complexity_vs_faithfulness.pdf}
    \caption{Complexity vs. faithfulness for different post-processing of both FreqRISE, LRP and IG relevance maps. }
    \label{fig:comp_vs_faith}
\end{figure}

Ideally both faithfulness and complexity scores should be low. Thus, an ideal explanation method would give results in the lower, left quadrant of the plot. From \autoref{fig:comp_vs_faith} it is clear that with existing methods, faithfulness and complexity are typically trade-offs of each other. 

For the digit task, FreqRISE consistently gives better faithfulness scores than the baselines independent of $p$. In the frequency domain, it is also clear that we are able to reduce complexity scores to a level closer to the best LRP complexity, while keeping a better faithfulness score (at $p=0.8$). In the time-frequency domain, we are able to lower the complexity, although not to a competitive level. However, here the gap in faithfulness between FreqRISE and competing methods is quite substantial, indicating that maybe a higher complexity is needed to properly describe the data. Additionally, it is worth mentioning that for both LRP and IG using only the positive values does not influence the faithfulness score much, but it does lower the complexity. 

For the gender task in the frequency domain, thresholds up to $p=0.6$ still gives better faithfulness scores than the full LRP and IG relevance maps. Additionally, the complexity score of FreqRISE is comparable or lower compared to both IG and LRP. Using the non-thresholded FreqRISE relevance map gives better faithfulness and comparable complexity to full LRP and IG relevance maps. If we use only the positive values of LRP and IG, the faithfulness score is worse than FreqRISE at all thresholds, but the complexity is lower. In the time-frequency domain FreqRISE generally performs worse on both faithfulness and complexity. This is discussed in the main paper. 

Generally, we see that with simple thresholding of the FreqRISE relevance maps, we are able to reduce complexity of FreqRISE relevance maps while keeping competitive faithfulness scores. 

\FloatBarrier

==> files/discussion.tex <==
\section{Discussion and conclusion}
Time series data is inherently difficult to interpret, due to the complex patterns of the signals \cite{rojat2021a}.
Therefore, providing relevance maps in a domain where information is sparser and more easily interpretable is desirable. 
We therefore proposed FreqRISE, which computes relevance maps in the frequency and time-frequency domains using model-agnostic masking methods. 
\citet{vilrp} previously produced relevance maps in these domains using gradient based methods, which are model-dependent, limiting the usability in cases where model gradients are not available. 

While LRP and IG are able to assign zero relevance, this is generally not the case for Freq(RISE). As a consequence, RISE and FreqRISE consistently yield high complexity scores. This is, however, not necessarily indicative of the perceptual quality of the relevance maps. The entropy could e.g. be reduced through post-processing of relevance maps. We have included preliminary results on a simple post-processing scheme in the appendix, showing that in most cases we can lower the complexity score to competitive levels while keeping a better faithfulness or localization score. Additionally, while complexity is a useful measure, it should always be considered in conjunction with localization and faithfulness scores. 

We used a synthetic dataset with known salient features in the frequency domain to compute localization scores. In the low noise setting, FreqRISE gave slightly higher accuracy in identifying the correct frequency components. However, when testing in the high noise setting, FreqRISE outperformed the two baseline methods by a large margin (100\% vs. 64\%). These results indicate that the gradient-based methods (IG and LRP) both are susceptible to noise in the data, which results in a lower localization score in the noisy setting. Clearly, FreqRISE does not suffer from the same issues and instead has a stable, high performance independent of the noise level - likely because it is not dependent on the gradients of the model.

On AudioMNIST, we measured the faithfulness of all methods across three domains. RISE performed either slightly worse or similar to the baseline methods in the time domain. However, in the frequency domain FreqRISE gave the best faithfulness scores. In the time-frequency domain, FreqRISE gave the best performance on the digit task, but the worst performance on the gender task. The difference is likely to be found in the different data properties of the two tasks. 
This leads us to believe that FreqRISE is most suitable for providing explanations in domains where the information is assumed to be sparse. While the same information can theoretically be found in e.g. the time domain, the intricacy of the patterns would require more advanced masking schemes to identify the same patterns. For the gender task, the frequency domain is sufficient for describing the data since the fundamental frequency is known to be discriminative of gender \cite{baken2000clinical}. Thus, when moving to the time-frequency domain, unnecessary complexity is added to the problem, resulting in a lower performance by FreqRISE. This leads us to believe that FreqRISE gives the best performance when computed in a domain where the salient information is sparse. As of now, no existing methods are able to estimate the "correct" domain in which to explain a model. Therefore, domain experts have to determine which domain is more useful for providing meaningful explanations. Future work should focus on developing metrics for measuring the most informative domains. 

Finally, like many other explainabilty methods, FreqRISE requires choosing a suitable set of hyper-parameters. This includes choosing an appropriate size of the lower dimensional grid on which we sample the binary masks, as well as the number of masks to use. As of now, we have no principled way of choosing these hyper-parameters, although one solution could be to tune the faithfulness and complexity scores on a small validation set. Another, less systematic approach, simply requires the user to estimate the granularity of the problem and choose the grid size based on this.  
FreqRISE requires a rather large number of masks ($N=10,000$) in order to produce high-quality relevance maps for AudioMNIST. This clearly increases the computational complexity compared to competing methods. Future work should investigate how to monitor convergence for potential early stopping. 

In conclusion, FreqRISE gives stable, good performance in localization and faithfulness on two different datasets with a total of 4 different tasks. Additionally, unlike existing methods, FreqRISE is completely model-independent requiring no access to gradients or weights of the models being explained. 
As such, FreqRISE is an important next step in providing robust explanations in the frequency and time-frequency domain for time series data. 
%We believe that XAI methods that can provide frequency and time-frequency relevance maps are important components in ensuring safe and trustworthy time series models. 



==> files/expsetup.tex <==
\section{Experimental setup} \label{sec:expsetup}
We conduct experiments on two datasets: the synthetic dataset presented in \cite{vilrp} and AudioMNIST \cite{audiomnist}. Both datasets have been shown to have salient information in either the frequency or time-frequency domain~\cite{vilrp}.
\subsection{Synthetic data}
We use the same synthetic dataset as in \cite{vilrp}. The dataset is specifically designed to have the salient information in the frequency domain and therefore allows us to test the localization ability of the XAI methods. Each data point is created as a sum over $J$ sinusoids. $J$ is sampled uniformly from $\mathcal{U}(10,50)$ :
\begin{equation}
    X_t = \sum_{j}^J a_j \sin\left(\frac{2\pi t}{T k_j} + \psi_j \right) + \epsilon.
\end{equation}
We set all $a_j = 1$, randomly sample the phase $\psi_j\sim\mathcal{U}(0, 2\pi)$, and add normally distributed noise $\epsilon\sim\mathcal{N}(0,\sigma)$. The length of the signals is set to $T=2560$ and all frequency components are sampled as integer values within the range $k_j\sim\mathcal{U}\{1, 59\}$. We train the models to detect a combination of frequencies, $k^*\in\{5, 16, 32, 53\}$ from the time series signal. The classes are created from the powerset of $k^*$ and we therefore have 16 classes. \autoref{fig:synthexample} shows a sample from the dataset.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/synthdataexample.pdf}
    \caption{A sample from the synthetic dataset with salient features at $k=\{5, 16, 53\}$ marked in blue in the frequency domain.}
    \label{fig:synthexample}
\end{figure}
We train a 4-layer multilayer perceptron (MLP) with a hidden size of 64 on two different versions of the raw time series: one with noise level $\sigma = 0.01$ and one with $\sigma = 0.8$. In both cases, we use $10^5$ samples for training. We test the models on a test set of size $1000$ with no noise. 

We use FreqRISE to compute relevance maps. We use the one-sided DFT to transform the signals to the frequency domain and sample binary masks, zeroing out single frequencies with $p=0.5$ from a Bernoulli distribution. Similar to recent work \cite{relax}, we use $N=3000$ masks to obtain relevance maps. 

\subsection{AudioMNIST}
AudioMNIST is a dataset consisting of 30,000 audio recordings of spoken digits (0-9) repeated 50 times for each of the 60 speakers (12 female/48 male) \cite{audiomnist}. We follow \cite{audiomnist} and downsample all signals to 8kHz and zero-pad all windows to 8000 samples. 

We use the same 1D convolutional architecture as in \cite{audiomnist} on the raw time series and train two versions: one for predicting the spoken digit and one to predict the gender of the speaker. Since the fundamental frequency is known to be discriminative for gender \cite{baken2000clinical}, we expect the salient information for the gender task to be localized in the frequency domain. The digit task, however, will likely be localized in both time and frequency, since we expect the numbers to be discriminated both through their formant information \cite{brend1990a} (frequency domain) and the ordering of these in time (time domain).

We use FreqRISE to compute relevance maps in the frequency and time-frequency domains and standard RISE in the time domain. We use 1000 data points from the gender and digit test sets respectively for testing the explanation methods. All relevance maps for AudioMNIST are estimated using $N=10,000$ sampled masks. All masks are sampled from a Bernoulli distribution with $p=0.5$ on a lower dimensional grid and linearly interpolated to create smooth masks. When computing the (Freq)RISE relevance maps, we use the logits prior to the softmax activation, since these show higher sensitivity to changes in the input. 

In the time-frequency domain, we use the one-sided STDFT with a Hanning window of size 455 and an overlap of 420 samples between subsequent windows following \cite{audiomnist}. In the STDFT domain, we use binary grids of size $25\times25$. In the time and frequency domains, we use grids of size $200$.

\subsection{Baselines}
As baselines, we use Integrated Gradients (IG) \cite{pmlr-v70-sundararajan17a} and Layer-wise Relevance Propagation (LRP) \cite{bach2015a}. When computing relevance maps in the frequency and time-frequency domains, we follow \cite{vilrp} and equip the models with virtual inspection layers, which map the input into the relevant domains. Due to relevance conservation, we are restricted to using rectangular, non-overlapping windows for the STDFT. We therefore use rectangular windows of size 455 with no overlap. 

\subsection{Quantitative evaluation}
\label{sec:quant}
Due to the lack of ground truth explanations \cite{hedstrom2023metaquantus}, quantitative evaluation for XAI is performed by measuring desirable properties \cite{hedstrom2023quantus}. Below we describe three such desirable properties that we use to quantify the quality of the relevance maps.

\textbf{Localization:} Localization scores are widely used to evaluate if explanations are co-located with a region of interest \cite{relax, dynamask}.
For the synthetic data, we know the ground truth explanations and can therefore use localization metrics to evaluate the methods. We use the \textit{relevance rank accuracy} \cite{clevr-xai}. Assuming a ground truth mask, $GT$, of size $K$ and a relevance map $\hat{\boldsymbol{R}}$, we take the $K$ points with the highest relevance. We then count how many of these values coincide with the positions in the ground truth mask. Formally, for $P_{top K} = \{p_1, p_2, \dots, p_K|\hat{R}_{p_1} > \hat{R}_{p_2} > \dots > \hat{R}_{p_K}\}$, i.e. $p$ denotes the position, we compute:
\begin{equation}
    \text{Relevance rank accuracy} = \frac{|P_{top K} \cap GT|}{|GT|}.
\end{equation}

\textbf{Faithfulness:} Faithfulness measures to what degree  an explanation follows the predictive behaviour of the model and is a widely used measure for quantifying quality of explanations \cite{vilrp, contralsp}. We follow prior works \cite{vilrp, dynamask} and compute faithfulness as follows. Given a relevance map, $\hat{\boldsymbol{R}}$, we iteratively remove the $5\%, 10\%, \dots, 95\%$ most important features by setting the signal value to 0. We then evaluate the model performance as the mean probability of the true class and plot it to produce deletion plots. Finally, we compute the area-under-the-curve (AUC) to produce our final faithfulness metric. A low AUC means that the explanation is faithful to the model.  

\textbf{Complexity:} Finally, we evaluate the complexity of the explanation as an estimate for the informativeness \cite{complexity}. The complexity is estimated as the Shannon entropy of the relevance maps. 


==> files/results.tex <==
\section{Results}
We present a comprehensive evaluation of FreqRISE using the experimental setup described in Section \ref{sec:expsetup}.
\subsection{Synthetic data results}
The two models trained on the synthetic dataset both achieve an accuracy of 100\%.
\autoref{tab:synth_res} shows the localization and complexity scores across the different methods for both the model trained on the low noise and the noisy datasets. The results on the low noise model show that all XAI methods perform approximately equal on the localization score, while IG and LRP yield relevance maps with substantially lower complexity scores compared to FreqRISE.
However, when we move to the noisy model, the localization score of FreqRISE is unchanged, whereas both IG and LRP have much lower performance. The complexity of the IG and LRP relevance maps is slightly higher on the noisy model, while the complexity of the FreqRISE is unchanged. An example of the computed relevance maps is shown in the appendix. 
\begin{table}[t]
    \centering
     \caption{Localization (L) and complexity (C) on the synthetic data.}
     \label{tab:synth_res}
    \begin{tabular}{lrrrr}
        \toprule
        & \multicolumn{2}{c}{Low noise} & \multicolumn{2}{c}{Noisy} \\
        \cmidrule(r){2-3}\cmidrule{4-5}
        & L ($\uparrow$) & C ($\downarrow$)  & L ($\uparrow$) & C ($\downarrow$) \\ \hline 
        IG & $99.1\%$ & $\mathbf{1.10}$ & $52.4\%$ & $1.96$\\
        LRP & $99.1\%$ & $1.11$ & $63.8\%$ & $\mathbf{1.34}$\\
        FreqRISE & $\mathbf{100.0\%}$  & $7.09$ & $\mathbf{100.0\%}$ & $7.09$ \\\bottomrule
    \end{tabular}
   
\end{table}

% \autoref{fig:synth_res} shows the explanations on the noisy model from each of the three methods on a sample in the test set. The figure again shows that RISE correctly identifies the four relevant frequencies, while IG and LRP indentify at most two of the ground truth frequencies. The plot also indicates the reason for the higher complexity of the RISE explanations compared to the LRP. While LRP and IG assigns no importance in regions with zero signal, RISE has a noisy baseline due to the computation. However, perceptually it is clear that even though RISE never assigns zero importance, the true relevance is presented as sharp peaks in the importance map.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figs/synthetic_highnoise.pdf}
%     \caption{Synthetic data: The plots show the DFT of one of the samples in the test set along with the ground truth explanations and the explanations provided by the three methods. If the explanation method assigns relevance in ground truth positions, the relevance is colored in blue, while explanations outside of the ground truth are colored in red.}
%     \label{fig:synth_res}
% \end{figure}

\subsection{AudioMNIST results}
%Subsequently, we compute results on the AudioMNIST tasks in the time, frequency and time-frequency domain.
The model trained on the digit classification task achieves and accuracy of 96.9\%, while the model trained on the gender tasks achieves an accuracy of 98.6\%.

Following the procedure described in Section \ref{sec:quant}, we initially compute the faithfulness results. \autoref{fig:digitdelet} (top) shows the deletion plots for the digit classification task in the frequency and time-frequency domain. We have also included two additional baselines, namely randomly deleting features (Rand.) and deleting features based on their amplitude (Amp.). 
In both domains, the mean true class probability quickly drops. After dropping only 10\% of the features, FreqRISE has a mean true class probability of $0.139$ in the time-frequency domain and $0.248$ in the frequency domain. 
After this, the value continues to drop with features being removed. 

\autoref{fig:digitdelet} (bottom) shows the same results for the gender classification task. Here, the mean true class probability using FreqRISE is $0.435$ after dropping only 5\% of the features in the frequency domain, and the same value in the time-frequency domain is $0.445$. The other methods drop to lower values in the time-frequency domain, indicating that FreqRISE struggles more to identify relevant features in the time-frequency domain. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/digit_gender_deletion.pdf}
    \caption{AudioMNIST: Deletion plots for both tasks in frequency and time-frequency domains. We delete features according to the importance and measure model outputs. FreqRISE outperforms the baselines in both domains on the digit task and the frequency domain on the gender task.}
    \label{fig:digitdelet}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figs/gender_stft_deletion.pdf}
%     \caption{AudioMNIST: Deletion plots for the gender task.}
%     \label{fig:genderdelet}
% \end{figure}

% \begin{table}[h]
%     \centering
%     %\small
%     \caption{AudioMNIST: Faithfulness of explanations in the time (T), frequency (F) and time-frequency (TF) domain.}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{lrrrrrr}
%          \toprule
%         & \multicolumn{3}{c}{Digit ($\downarrow$)} & \multicolumn{3}{c}{Gender ($\downarrow$)} \\
%         \cmidrule(r){2-4}\cmidrule{5-7}
%         & T & F  & TF & T & F  & TF \\ \hline 
%         IG & $.183$ & $.251$ & $.194 $& $.470$ & $.428$ & $\mathbf{.389}$ \\
%         LRP & $\mathbf{.168}$ & $.204$ & $.209$ & $.401$ & $.431$ & $.420$\\
%         (Freq)RISE & $.212$ & $\mathbf{.147}$  & $\mathbf{.124}$ & $\mathbf{.399}$ & $\mathbf{.414}$ & $.522$\\\bottomrule
%     \end{tabular}
%     }
%     \label{tab:audio_sdf}
% \end{table}


In \autoref{tab:audio_res} (top), the faithfulness scores are shown for both models in all three domains. We notice that in the time domain, RISE performs either worse or equivalently compared to LRP. However, when we move to the frequency domain, the faithfulness scores are lowest for FreqRISE in both cases. Finally, when we look at the time-frequency domain, the faithfulness score increases for FreqRISE on the gender task, while it decreases on the digit task. These results indicate that the information is sparser for the digit task in the time-frequency domain.

\autoref{tab:audio_res} (bottom) shows the complexity scores across all methods, domains and tasks. Again, it is clear that the complexity of the masking based methods is higher compared to the remaining methods. 


% \begin{table}[t]
%     \centering
%     \caption{AudioMNIST: Faithfulness (Faith.) and Complexity (Comp.) scores for explanations in the time (T), frequency (F), and time-frequency (TF) domains.}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l l r r r r r r r}
%         \toprule
%         & & \multicolumn{3}{c}{Digit ($\downarrow$)} & \multicolumn{3}{c}{Gender ($\downarrow$)} \\
%         \cmidrule(r){3-5}\cmidrule{6-8}
%         Metric & Method & T & F & TF & T & F & TF \\ \hline 
%         \multirow{3}{*}{Faith.} 
%         & IG & $.183$ & $.251$ & $.194$ & $.470$ & $.428$ & $\mathbf{.389}$ \\
%         & LRP & $\mathbf{.168}$ & $.204$ & $.209$ & $.401$ & $.431$ & $.420$ \\
%         & (Freq)RISE & $.212$ & $\mathbf{.147}$ & $\mathbf{.124}$ & $\mathbf{.399}$ & $\mathbf{.414}$ & $.522$ \\ \hline
%         \multirow{3}{*}{Comp.} 
%         & IG & $6.93$ & $6.41$ & $5.26$ & $\mathbf{6.57}$ & $\mathbf{4.74}$ & $\mathbf{4.04}$ \\
%         & LRP & $\mathbf{6.88}$ & $\mathbf{5.84}$ & $\mathbf{4.67}$ & $6.78$ & $5.16$ & $4.16$ \\
%         & (Freq)RISE & $8.86$ & $8.17$ & $10.82$ & $8.86$ & $8.01$ & $10.78$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:audio_combined}
% \end{table}
% \begin{table}[t]
%     \centering
%     %\small
%     \caption{AudioMNIST: Faithfulness of explanations in the time (T), frequency (F) and time-frequency (TF) domain.}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{lrrrrrr}
%          \toprule
%         & \multicolumn{3}{c}{Digit ($\downarrow$)} & \multicolumn{3}{c}{Gender ($\downarrow$)} \\
%         \cmidrule(r){2-4}\cmidrule{5-7}
%         & T & F  & TF & T & F  & TF \\ \hline 
%         IG & $.183$ & $.251$ & $.194 $& $.470$ & $.428$ & $\mathbf{.389}$ \\
%         LRP & $\mathbf{.168}$ & $.204$ & $.209$ & $.401$ & $.431$ & $.420$\\
%         (Freq)RISE & $.212$ & $\mathbf{.147}$  & $\mathbf{.124}$ & $\mathbf{.399}$ & $\mathbf{.414}$ & $.522$\\\bottomrule
%     \end{tabular}
%     }
%     \label{tab:audio_sdf}
% \end{table}
\begin{table}[t]
    \centering

    %\small
        \caption{AudioMNIST: Faithfulness (top) and Complexity (bottom) scores for explanations in the time (T), frequency (F) and time-frequency (TF) domains.}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrrrrr}
        \toprule
        & \multicolumn{3}{c}{Digit ($\downarrow$)} & \multicolumn{3}{c}{Gender ($\downarrow$)} \\
        \cmidrule(r){2-4}\cmidrule{5-7}
        & T & F  & TF & T & F  & TF \\ \hline 
        IG & $.183$ & $.252$ & $.197 $& $.470$ & $.428$ & $\mathbf{.389}$ \\
        LRP & $\mathbf{.168}$ & $.205$ & $.214$ & $\mathbf{.401}$ & $.431$ & $.420$\\
        (Freq)RISE & $.233$ & $\mathbf{.160}$  & $\mathbf{.104}$ & $.419$ & $\mathbf{.416}$ & $.423$\\\bottomrule
        \toprule
        & \multicolumn{3}{c}{Digit ($\downarrow$)} & \multicolumn{3}{c}{Gender ($\downarrow$)} \\
        \cmidrule(r){2-4}\cmidrule{5-7}
        & T & F  & TF & T & F  & TF \\ \hline 
        IG & $6.93$ & $6.41$ & $5.26$ & $\mathbf{6.57}$ & $\mathbf{4.74}$ & $\mathbf{4.04}$ \\
        LRP & $\mathbf{6.88}$ & $\mathbf{5.84}$ &  $\mathbf{4.67}$ & $6.78$ & $5.16$ & $4.16$ \\
        (Freq)RISE & $8.86$ & $8.17$  & $10.82$ & $8.86$ & $8.01$ & $10.78$\\\bottomrule
    \end{tabular}
    }
    \label{tab:audio_res}
    
\end{table}

% \begin{table}[h]
%     \centering
%     \caption{AudioMNIST: Faithfulness and Complexity scores for explanations in the time (T), frequency (F), and time-frequency (TF) domains.}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l r r r r r r r}
%         \toprule
%         & \multicolumn{3}{c}{Digit ($\downarrow$)} & \multicolumn{3}{c}{Gender ($\downarrow$)} \\
%         \cmidrule(r){2-4}\cmidrule{5-7}
%         Method & T & F & TF & T & F & TF \\ \midrule 
%         \multicolumn{7}{c}{\textbf{Faithfulness}} \\ \midrule
%         IG & $.183$ & $.251$ & $.194$ & $.470$ & $.428$ & $\mathbf{.389}$ \\
%         LRP & $\mathbf{.168}$ & $.204$ & $.209$ & $.401$ & $.431$ & $.420$ \\
%         (Freq)RISE & $.212$ & $\mathbf{.147}$ & $\mathbf{.124}$ & $\mathbf{.399}$ & $\mathbf{.414}$ & $.522$ \\ \hline
%         \multicolumn{7}{c}{\textbf{Complexity}} \\ \midrule
%         IG & $6.93$ & $6.41$ & $5.26$ & $\mathbf{6.57}$ & $\mathbf{4.74}$ & $\mathbf{4.04}$ \\
%         LRP & $\mathbf{6.88}$ & $\mathbf{5.84}$ & $\mathbf{4.67}$ & $6.78$ & $5.16$ & $4.16$ \\
%         (Freq)RISE & $8.86$ & $8.17$ & $10.82$ & $8.86$ & $8.01$ & $10.78$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:audio_combined}
% \end{table}

\begin{figure}[t]
     \centering

         \includegraphics[width=\linewidth]{figs/audionet_gender_0_700.png}
         \caption{AudioMNIST: Gender task. We show relevance maps computed by LRP and FreqRISE in the time and frequency domain. The salient information is more localized in the frequency domain.}
         \label{fig:gender}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/stft_digit_9.pdf}
    \caption{AudioMNIST: Digit task. STDFT of the signal on the left and the FreqRISE relevance map in the time-frequency domain on the right. The relevance map shows the benefit of having both the time and frequency axis, when the describing the digit data.}
    \label{fig:dig_stft}
\end{figure}

\autoref{fig:gender} (top) shows an example of relevance maps computed in the time domain on the gender classification task. \autoref{fig:gender} (bottom) shows the same sample in the frequency domain. The sample is from a female speaker and the model correctly predicts the class. We see that LRP has a very sparse but scattered signal in the time domain, while RISE appears very noisy. Moving to the frequency domain, the relevance is much more localized, with FreqRISE putting most emphasis on the fundamental frequency, while LRP also focuses on the harmonics. The fundamental frequency is known to be discriminative of gender \cite{baken2000clinical}. 

\autoref{fig:dig_stft} shows the relevance map computed using FreqRISE in the time-frequency domain for the digit task. The spoken and predicted digit is 9. The STDFT reveals that the signal starts around $t=0.3s$, where the relevance map puts most of the relevance. However, around $t=0.5s$, there are two distinct patterns emerging along the frequency axis. The fact that the method is allowed to distribute the relevance differently across frequencies depending on the time shows the benefit of having both the time and frequency component when computing relevance maps for the digit task. 

